Graph Spectral Feature Learning for Mixed Data of Categorical and Numerical Type

Feature learning in the presence of a mixed type of variables, numerical and categorical types, is an important issue for related modeling problems. For simple neighborhood queries under mixed data space, standard practice is to consider numerical and categorical variables separately and combining them based on some suitable distance functions. Alternatives, such as Kernel learning or Principal Component do not explicitly consider the inter-dependence structure among the mixed type of variables. In this work, we propose a novel strategy to explicitly model the probabilistic dependence structure among the mixed type of variables by an undirected graph. Spectral decomposition of the graph Laplacian provides the desired feature transformation. The Eigen spectrum of the transformed feature space shows increased separability and more prominent clusterability among the observations. The main novelty of our paper lies in capturing interactions of the mixed feature type in an unsupervised framework using a graphical model. We numerically validate the implications of the feature learning strategy

==> IEEE Bare Demo Template for Conferences (3)/list_of_references.tex <==

%noisy feature removal 
3. Han J. Data Mining: Concepts and Techniques. San Francisco, Calif, USA: Morgan Kaufmann Publishers; 2005.

4. Strong D. M., Lee Y. W., Wang R. Y. Data quality in context. Communications of the ACM. 1997;40(5):103?110.


% similarity based agglomerative
[5] C. Li and G. Biswas, ??Unsupervised learning with mixed numeric and nominal data,?? IEEE Trans. Knowl. Data Eng., vol. 14, no. 4,
pp. 673?690, Jul./Aug. 2002.
%PAM
[21] Kaufman, L. and Rousseeuw, P.J. (1987), Clustering by means of Medoids, in Statistical Data
Analysis Based on the L1 - Norm and Related Methods, edited by Y. Dodge, North- Holland, 405?
416.
%proto
Huang, Z. Clustering large data sets with mixed numeric and categorical values. In Proceedings of the First Pacific Asia Knowledge Discovery and Data Mining Conference, Singapore, 23?24 February 1997; pp. 21?34.
 %ensemble
 [9] Z. He, X. Xu, and S. Deng. (2005). ??Clustering mixed numeric and
categorical data: A cluster ensemble approach.?? [Online]. Available:
http://arxiv.org/abs/cs/0509011




%pca
1. Pearson K. On lines and planes of closest fit to systems of points in space. Philos Mag. 1901;2:559e572.
%isomap
5. Tenenbaum J, Silva V, Langford J. A global geometric framework for nonlinear dimensionality reduction. Science. 2000;290:2319e2323. 6. Roweis S, Saul L. Nonlinear dimensionality reduction by locally linear embedding. Science. 2000;290:2323e2326.
%lle
6. Roweis S, Saul L. Nonlinear dimensionality reduction by locally linear embedding. Science. 2000;290:2323e2326.
%graph
23. Yan S, Xu D, Zhang B, Zhang H-J, Yan Q, Lin S. Graph embedding and extensions: a general framework for dimensionality reduction. IEEE
Trans Pattern Anal Mach Intell. 2007;29:40e51.
%MDS
29. Cox T, Cox M. Multidimensional Scaling. Boca Raton: Chapman and Hall; 2001.
%KPCA
31. Sch¤olkopf B, Smola A, Muller K-R. Nonlinear component analysis as a kernel eigenvalue problem. Neural Comput. 1998;10:1299e1319.

%DL
15. Bengio Y, Lamblin P, Popovici D, Larochelle H. Greedy layer-wise training of deep networks. In: NIPS. 2006:153e160.
%SVD
30. Dumais S. Latent semantic analysis. ARIST. 2004;38:188e230.


%diffusion
Ahn, Jeongyoun, et al. ?The High-Dimension, Low-Sample-Size Geometric Representation Holds under Mild Conditions.? Vol. 94, no. 3, 2007, pp. 760?766. JSTOR, www.jstor.org/stable/20441411. Accessed 23 Feb. 2019.
%J
Wang, L. & Chan, K. Luk. (2002). Learning kernel parameters by using class separability measure. The sixth kernel machines workshop, in conjunction with Neural Information Processing Systems (NIPS) (pp. 1-8).

%rand index
Rand, W.M. 1971. Objective criteria for the evaluation of clustering methods. Journal of the American Statistical Association 66: 846--850. Hubert, L. and Arabie, P. 1985. Comparing partitions. Journal of Classification. 2: 193--218.




==> list_of_references.tex <==

%noisy feature removal 
3. Han J. Data Mining: Concepts and Techniques. San Francisco, Calif, USA: Morgan Kaufmann Publishers; 2005.

4. Strong D. M., Lee Y. W., Wang R. Y. Data quality in context. Communications of the ACM. 1997;40(5):103?110.


% similarity based agglomerative
[5] C. Li and G. Biswas, ??Unsupervised learning with mixed numeric and nominal data,?? IEEE Trans. Knowl. Data Eng., vol. 14, no. 4,
pp. 673?690, Jul./Aug. 2002.
%PAM
[21] Kaufman, L. and Rousseeuw, P.J. (1987), Clustering by means of Medoids, in Statistical Data
Analysis Based on the L1 - Norm and Related Methods, edited by Y. Dodge, North- Holland, 405?
416.
%proto
Huang, Z. Clustering large data sets with mixed numeric and categorical values. In Proceedings of the First Pacific Asia Knowledge Discovery and Data Mining Conference, Singapore, 23?24 February 1997; pp. 21?34.
 %ensemble
 [9] Z. He, X. Xu, and S. Deng. (2005). ??Clustering mixed numeric and
categorical data: A cluster ensemble approach.?? [Online]. Available:
http://arxiv.org/abs/cs/0509011




%pca
1. Pearson K. On lines and planes of closest fit to systems of points in space. Philos Mag. 1901;2:559e572.
%isomap
5. Tenenbaum J, Silva V, Langford J. A global geometric framework for nonlinear dimensionality reduction. Science. 2000;290:2319e2323. 6. Roweis S, Saul L. Nonlinear dimensionality reduction by locally linear embedding. Science. 2000;290:2323e2326.
%lle
6. Roweis S, Saul L. Nonlinear dimensionality reduction by locally linear embedding. Science. 2000;290:2323e2326.
%graph
23. Yan S, Xu D, Zhang B, Zhang H-J, Yan Q, Lin S. Graph embedding and extensions: a general framework for dimensionality reduction. IEEE
Trans Pattern Anal Mach Intell. 2007;29:40e51.
%MDS
29. Cox T, Cox M. Multidimensional Scaling. Boca Raton: Chapman and Hall; 2001.
%KPCA
31. Sch¤olkopf B, Smola A, Muller K-R. Nonlinear component analysis as a kernel eigenvalue problem. Neural Comput. 1998;10:1299e1319.

%DL
15. Bengio Y, Lamblin P, Popovici D, Larochelle H. Greedy layer-wise training of deep networks. In: NIPS. 2006:153e160.
%SVD
30. Dumais S. Latent semantic analysis. ARIST. 2004;38:188e230.


%diffusion
Ahn, Jeongyoun, et al. ?The High-Dimension, Low-Sample-Size Geometric Representation Holds under Mild Conditions.? Vol. 94, no. 3, 2007, pp. 760?766. JSTOR, www.jstor.org/stable/20441411. Accessed 23 Feb. 2019.
%J
Wang, L. & Chan, K. Luk. (2002). Learning kernel parameters by using class separability measure. The sixth kernel machines workshop, in conjunction with Neural Information Processing Systems (NIPS) (pp. 1-8).

%rand index
Rand, W.M. 1971. Objective criteria for the evaluation of clustering methods. Journal of the American Statistical Association 66: 846--850. Hubert, L. and Arabie, P. 1985. Comparing partitions. Journal of Classification. 2: 193--218.



